Normal-guided Garment UV Prediction for Human Re-texturing

Clothes undergo complex geometric deformations, which lead to appearance changes. To edit human videos in a physically plausible way, a texture map must take into account not only the garment transformation induced by the body movements and clothes fitting, but also its 3D fine-grained surface geometry. This poses, however, a new challenge of 3D reconstruction of dynamic clothes from an image or a video. In this paper, we show that it is possible to edit dressed human images and videos without 3D reconstruction. We estimate a geometry aware texture map between the garment region in an image and the texture space, a.k.a, UV map. Our UV map is designed to preserve isometry with respect to the underlying 3D surface by making use of the 3D surface normals predicted from the image. Our approach captures the underlying geometry of the garment in a self-supervised way, requiring no ground truth annotation of UV maps and can be readily extended to predict temporally coherent UV maps. We demonstrate that our method outperforms the state-of-the-art human UV map estimation approaches on both real and synthetic data.

==> cvpr_intro2.tex <==
\section{Introduction}

% \yasamin{1. I want to talk about the goal here: My goal is to have appearance/texture editing of a garment from an image of human. for example I want to change my dress texture to a color and pattern that goes better with my face, or I want to insert my company or school Logo on top f my Tshirt in a realistic manner}

While browsing online clothing shops, have you ever wondered how the appearance of an item of interest would look on you as if you were in a fitting room? 
A key technology to enable generating such visual experiences is \textit{photorealistic re-texturing}---editing the texture of clothes in response to the subject's movement in the presented images or videos in a geometrically and temporally coherent way.
Over the past few years, there has been a significant advancement in the image and video editing technologies \cite{ling2021editgan, wu2020cascade, Navigan_CVPR_2021, shen2020interpreting, bau2019semantic, chen2020deepfacedrawing, alharbi2020disentangled, collins2020editing, kim2021stylemapgan, lee2020maskgan, hou2020guidedstyle, he2019attgan}, such as inserting advertising logos on videos of moving cars or applying face makeup on social media. 
However, such editing approaches designed for rigid or semi-rigid surfaces are not suitable for garments that undergo complex secondary motion with respect to the underlying body. For example, the fine wrinkles of the dress in Figure \ref{fig:teaser} result in complex warps in texture over time. 
In this paper, we present a new method to edit the appearance of a garment in a given image or video by taking into account its fine-grained geometric deformation. 
% editing videos and images gets more complicated when dealing with dynamic objects such as garments. 
%%%%%%%%%%%%%%%%%%%%%%for later%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The two biggest obstacles to editing dressed human images and videos in a physically realistic way are as follows: intricate geometry of clothes, and complex secondary dynamics, which leads to the unrealistic rendering of the garments.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \yasamin{2. I want to talk about the challenge here.  technical challenges of existing work (requiring 3D reconstruction). to be able to do the above, I need to have a representative geometry either by having a 3D mesh or By having a geometry-aware UV so we can bypass the 3D reconstruction requirement. }
Previous works address photorealistic texture editing in two ways. (1) 3D reconstruction and rendering: 
% \yi{They first reconstruct the 3D geometry, then map the texture uv onto the surface and render the texture by uv mapping.}
%given a 3D model is it possible to map the texture onto the surface and use texture mapping to render the warped texture onto the image plane.  
\yi{This type of approaches can achieve high-fidelity texture editing if the given 3D geometry has high accuracy. However, on other side of the coin, their performance is highly limited by the quality of the 3D reconstruction. While the garment's 3D geometry can be learned from paired human appearance data, e.g., human modeling repositories with 3D meshes and renderings~\cite{RP:2020}, due to the scarcity of such data, it often cannot generalize well on unseen real images and videos.}
% (a few hundred models, limited range of poses and appearances, and lack of complex fabric geometry) often leads to limited generalization on unseen real images and videos
%The quality of the rendered image is governed in large part by the geometric accuracy of the 3D mesh, and therefore, high-fidelity texture editing is possible given a high quality 3D mesh model. The core challenge 
 % of this approach lies in the limited ability to reconstruct the underlying 3D geometry of the garment from a single image or video. This challenge can be addressed by learning 3D meshes from paired human appearance data, e.g., 3D mesh models from human modeling repositories~\cite{RP:2020} with their rendered images. Nonetheless, scarcity of such data (a few hundred models, limited range of poses and appearances, and lack of complex fabric geometry) often leads to limited generalization on unseen real images and videos. 
(2) Direct texture mapping: 
%direct texture map of an image, or UV map, 
\yi{By estimating dense uv correspondences, this type of methods can bypass the procedure of 3D reconstruction and are widely used on human bodies~\cite{guler2018densepose, Neverova2020ContinuousSurfaceEmbeddings, Neverova2021UniversalCanonicalMaps, ianina2022bodymap, Xie_2022_CVPR}. However, they usually lack of details and only capture the underlying human body, thus, not applicable for editing garments. Moreover, when applied to videos, such methods will produce much more salient visual artifacts since they do not capture the underlying deformation of the garment's 3D geometry \cite{kasten2021layered,ye2022sprites
}}
%For instance, with estimated human dense correspondences~\cite{guler2018densepose, Neverova2020ContinuousSurfaceEmbeddings, Neverova2021UniversalCanonicalMaps, ianina2022bodymap, Xie_2022_CVPR}, one can directly map the texture to the image. 
%However, these UV estimations are not applicable for editing garments because of their lack of details, i.e., the estimated UV maps only capture the underlying body shape. Hence, when applied to a video, such methods will produce much more salient visual artifacts since they do not capture the underlying deformation of the garment's 3D geometry \cite{kasten2021layered,ye2022sprites}. 

% This challenge can be addressed by obtaining a 3D mesh from the image or a temporally coherent 3D mesh from the video. 
% However, to perform such reconstruction, high-fidelity 3D models of humans must be used as the ground truth to learn from the images, and videos \cite{pifu:2019, pifuhd:2020}. 
% Nevertheless, because of the restricted availability of such data, which cover a limited range of poses, appearances, or complex fabric geometry, these 3D human reconstruction approaches fail when used with real-world images and videos.
% The requirement of 3D reconstruction can be avoided by leveraging the 2D dense correspondences (UV maps) instead to edit dressed human photos and videos in a physically plausible manner.


% \yasamin{3. Now I want to talk about the existing methods in UV estimation. I have the naked body methods like densepose..., they have 2 problems: they don't represent clothing boundary also as they are trained on the naked body they don't represent the local geometry. Then we have hgps, bodymap that use a limited amount of 3D mesh to predict the full-dressed body but they are not representative of the local geometry because of 2 reasons (1)they don't specifically enforce the local geometry to be preserved (2) they use synthetic data that is very different from the real world imagery, so that is why they don't perform well on the real world images in preserving the local geometry. Then we have neural atlas and deformable sprites that decompose the video to fg and bg UV maps. There is 2 problem with these methods: (1) they can only be applied on a video and they cannot be applied to a single image.  (2) They can provide some coarse deformation of the UV for example motion of the arm or legs in the sequence but they fail for smaller deformations like clothe wrinkles.}





% To obtain such UV maps, previous methods on Human UV estimation \cite{guler2018densepose, Neverova2020ContinuousSurfaceEmbeddings, Neverova2021UniversalCanonicalMaps, ianina2022bodymap, Xie_2022_CVPR} learn dense human UV coordinates from the ground truth data fitted on the underlying naked human body. Therefore, these methods are unsuitable for editing garments' appearance as they do not capture the fine-grained surface geometry. 
% Video-based UV estimation approaches \cite{kasten2021layered,ye2022sprites} decouple the video to estimate a foreground and a background UV map based on the motion captured in the frames. 
% However, while they can produce coarse UV deformations, such as arm or leg movements during a sequence, they fall short for micro deformations like wrinkles in the clothing. Furthermore, these techniques cannot represent UV mapping for an image and can only be used for videos.

% \yasamin{4. in this paper, we propose a high-fidelity UV estimation that can be used both for images and videos of dressed humans. We use the geometric correlation between the surface normal and garment UV coordinates to get the details of the surface. We also apply temporal consistency to achieve high-fidelity UVs that are temporally coherent in a video.}

% In this paper, we propose a high-fidelity UV estimation of garments that can be applied to images and videos of dressed humans.

Our method is designed to enjoy the advantages of both two approaches: 
\yi{preserving realistic details while circumventing 3D reconstruction.}
%direct UV map estimation without 3D reconstruction while preserving 3D geometric details. 
% \nate{ Our method follows only the second approach (i.e. we compute a uv mapping without explicit 3D geometry).   
% The key insight is we impose fundamental geometric properties in the uv mapping process derived from surface normals(which are more robust to estimate than 3D geometry). This leads to higher quality results without needing to infer full 3D information. }
To achieve this, we formulate a new isometric UV parametrization that takes into account a fundamental geometric property called isometry via 3D surface normals. 
The resulting UV map preserves length and angle avoiding stretching artifacts. This optimization is conducted in a self-supervised manner, i.e., it requires no additional ground truth UV map or 3D data.
We generalize our method for videos by making use of optical flow %\cite{LucasK81, LucasK85} to achieve temporal coherence across frames.

% We employ a novel formulation to utilize surface normal in predicting UV coordinates by preserving the conformality (angle) and isometry (length) concerning the underlying 3D surface without using any ground truth information.
% Additionally, we make use of Optical Flow tracking \cite{LucasK81,LucasK85} to achieve temporal coherence across the course of a video.

% \yasamin{5. For the processing of an image, we first get an initial UV using an extrapolation of DensePose. Then we train an MLP where the input is xy location of the pixels of a garment (segmented using \cite{Gong2019Graphonomy}) and the output is the uv location. Then we optimize the pediction UV area to be close to the extrapolated densepose and also we make sure that the surface normal-uv consistency is preserved. }


Our method takes as input an image or video, its surface normal prediction, and dense optical flow (optionally for video), and outputs the geometry aware UV map estimate. 
The UV map is modeled by a multi-layer perceptron that can predict the UV coordinates given a pixel location in an image, which is constrained by the partial differential equation provided by isometry. 
% We note that the UV map is defined up to the choice of a reference coordinate frame. To disambiguate this, 
We condition the neural network with a pre-defined proxy UV map (e.g., DensePose~\cite{guler2018densepose}) to disambiguate the coordinate system. 
% We use the isometry constraints as a loss to optimize the UV map.
% \duygu{do we use per-pixel features or per-frame features?} 
Further, for a video, we leverage the per-frame image feature to correlate the UV coordinates of the pixels across time using optical flow.

% For predicting the high-fidelity UV of a garment from an image, we train a Multi-Layer-Perceptron (MLP) where the input is the XY location of a pixel inside the garment, and the output is the corresponding UV coordinate.
% We initialize the MLP with a regularization term to fit the prediction to a coarse UV generated by the DensePose \cite{guler2018densepose}. Since the UV map from DensePose contains various body parts, we select the most representative body part for each garment (for example, the torso for dresses and T-shirts and the upper right leg for skirts). We then use a simple extrapolation \cite{Telea_inpaint} on to chosen body part UV to obtain an initial UV coordinate for all the pixels in the garment segmentation \cite{Gong2019Graphonomy}.
% We further enforce the predicted UV to preserve the conformality (angle) and isometry (length) information captured in a surface normal prediction of the garment \cite{Jafarian_2021_CVPR_TikTok}.


% \yasamin{6. for processing a video, we extract the optical flow beforehand between the adjacent frames and train one MLP for all the frames of a sequence. to make sure the MLP can differentiate between the different frames, we also extract an image feature using a resnet backbone. now this feature vector with the xy is fed to the MLP and the output is uv coordinate for that pixel. here we not only enforce the consistency between UV and normal and UV and extrapolated densepose, we also apply the consistency between the adjacent frames such that they should satisfy the flow captured in the optical flow computation.}

% For high-fidelity UV prediction of a garment from a video, we train the MLP for all the frames together. 
% To confirm that the MLP can distinguish between the various frames, we also extract an image feature with the help of a ResNet-152 \cite{He_2016_CVPR_resnet} backbone, which is then concatenated with the XY pixel location as the input to the MLP.
% In the video training process, we not only enforce the geometric consistency between UV and surface normal and the UV regularization term, but we also apply the consistency between the adjacent frames to satisfy the flow captured in the Optical Flow computation \cite{LucasK81,LucasK85}.

% \yasamin{7. My contributions are}

We present three core contributions: 
(1) a novel formulation that captures the geometric relationship between the 3D surface normals and UV map by preserving the isometry, which eliminates the requirement of 3D reconstruction and ground truth UV map;
(2) a neural network design that learns to predict temporally coherent UV map for the frames by correlating per-frame image features; 
(3) stronger performance 
% \nate{ are we only competitive? Can we say "better performance in capturing fine detail"? } 
than the previous existing re-texturing methods and compelling results on a wide range of real-world imagery.


% We present three core contributions: 
% (1) a novel formulation that captures the geometric correlation between the surface normal and UV coordinates by maintaining the conformality (angle) and isometry (length), which allows us to utilize authentic human images and videos without any use of ground truth; 
% (2) a design that learns to predict temporally coherent UV coordinates for the frames of a video by encoding each one by the corresponding image feature; 
% (3) strong qualitative and quantitative prediction on real-world imagery.

==> cvpr_intro_temp.tex <==
Consider the historical painting "The School of Athens" by Raffaello Sanzio da Urbino (1509–1511) in Figure \ref{fig:teaser}, showing garments with detailed clothing geometry including wrinkles and folds which we as humans can effortlessly perceive from this 2D painting. 
Can a machine have the vision necessary to provide the precise geometry of these garments, allowing us to replace the textures with modern fashion patterns or insert a logo into this depiction while being faithful to the geometry?
Additionally, take into account this dance video from TikTok (Figure \ref{fig:teaser}). Can we replace the textures in all the frames such that they are both faithful to geometry and coherent across time? 
Building dense correspondences between human images can enable this perceptual ability to perfectly model the intricate geometry of humans and their temporal consistency, which is the key to real social telepresence, virtual clothes try-on, non-rigid tracking, appearance transfer, image/video editing, and augmented reality. 

In the clothing industry, to insert the company logo on top of the model photos, usually photoshop designers obtain a dense correspondence map by starting from a plain UV layer and manually tweak it to represent the wrinkles and folds of the clothing. However, this process is not automated and it only applies to one image and there will be no correspondences between frames of a sequence or different subjects. To address this challenge previous methods \cite{} train a neural network using ground truth UV maps. HumanGPS \cite{tan2021humangps} uses 3D mesh models to render UV maps of full human body. However, as our task specifies each garment type, it needs 3D ground truth with consistent UV unwrapping for similar garments (e.g. a Tshirt for different subjects), which such data does not exist and needs manual annotation to capture the ground truth. Nonetheless, there are only a small number of these 3D data available to train such a model (a few hundred static models, for example), and because they do not cover a wide range of poses, appearances, and complex cloth geometry, they degrade the performance of human UV generation when used with real-world imagery. Other methods \cite{guler2018densepose, Neverova2020ContinuousSurfaceEmbeddings, Neverova2021UniversalCanonicalMaps} Use the naked human models to learn a consistent UV across all instances, however these methods do not represent the clothing and local geometries (e.g. clothes wrinkles).

\textbf{Second paragraph}\\
% In this paper, …
% Insight: why this would work
% How this solution can overcome the challenges 
In this paper, we fill this data gap by utilizing a new geometry-aware supervision between surface normal and UV to achieve high-fidelity UV estimation. In addition, we utilize optical flow tracking to obtain the temporal coherence throughout the duration of a video. To achieve this goal we start from a coarse UV estimation (e.g. DensePose) and garment segmentation \cite{Gong2019Graphonomy}, where for each garment we extrapolate the UV of that body part to fill the garment mask which provides us with an initial UV. We then enforce the geometric consistency between surface normal prediction \cite{Jafarian_2021_CVPR_TikTok} and UV to refine the initial UV. To ensure that the prediction is temporally coherent we also impose the optical flow consistency between adjacent frames.

==> cvpr_intro_temp2.tex <==
\section{Introduction}
\textbf{First paragraph}:\\
% Motivation and problem identification
% Limitation of existing solution
% Why challenging?
% Posing research questions

% challenge: no geo and clothes-aware UV out there, the UVs out there are not aligned with garments. No such data exist. 

While browsing clothing online shops, Have you ever wondered how the texture of an item of interest, would look on you while moving around to see yourself from different views? How can we edit the appearance of human videos in a geometric and temporally plausible manner without the need to reconstruct the 3D representation? \jimei{It'd be good to call out the general research challenges of editing human images and videos in term of garments and also point out a few applications including the one above. Why no need for 3D reconstruction?} To answer this question, we can achieve modifying the appearance of the garments (such as swapping the texture or adding a logo in a convincing way) by having a geometry-aware and temporally consistent Dense Correspondence (DC) map. The two biggest obstacles to editing human footage in a way that is physically realistic are as follows: intricate geometry of clothes, and complex secondary dynamics, which leads to the unrealistic rendering of the garments.

% In the modern age of technology, AR pushes the boundary of the fashion industry, enabling virtual try-on that allow remote buyers to see themselves as if they wear the items of interest. However, so far, the virtual try-on that is actually used on shopping websites is limited to a few items placed on the face and head e.g., makeup, sunglasses, and wigs. These items are rendered on the limited face and head movements. 
% On the other hand, for clothes like dresses, due to technical challenges, the virtual try-on applies only to pre-defined static poses. This contrasts sharply with how we try on a dress in the store as we move ourselves to see how it fits and how the garment patterns look as they go under complex motions. 
% The main challenges of achieving the dress virtual try-on are two folds: complex geometry of clothes, and complex secondary dynamics, which leads to the unrealistic rendering of the garments.

% In the clothing industry, to obtain such a try-on with the model photos, usually, photoshop designers obtain a dense correspondence map by starting from a plain UV layer and manually tweaking it to represent the wrinkles and folds of the clothing. By obtaining this UV layer, they can then swap the texture of the garments in a realistic manner. However, this process is not automated and it only applies to a few images of the models uploaded on the shopping websites and is not available to everyone else as there will be no correspondences between frames of a sequence or different subjects. 
To address this challenge, previous methods \cite{tan2021humangps,guler2018densepose,Neverova2020ContinuousSurfaceEmbeddings} train a neural network using ground truth DC maps. \jimei{using a 3D template as a reference} However, such available datasets to train a DC estimator are either for naked human body \cite{guler2018densepose,Neverova2020ContinuousSurfaceEmbeddings} and not representative of clothing or a few hundred limited clothed 3D meshes \cite{tan2021humangps} \jimei{do you mean "limited by a few ..."?}, which when used to real-world photos do not cover a wide range of poses, looks, and intricate fabric geometry, causing UV \jimei{you have been using DC map instead of UV above. Better to formulate a bit better} estimation reconstruction to perform poorly.

\jimei{It can be better to clarify the relationship between dense correspondences and UV mapping.}


\textbf{Second paragraph}:

In this paper, we learn a high-fidelity garment-specific, geometry-aligned, DC prediction paradigm by utilizing a novel geometry-aware supervision between the surface normal and DC coordinates \jimei{it is not clear what DC coordinates mean} without any use of ground truth. In addition, we utilize optical flow tracking to obtain temporal coherence throughout the duration of a video. To achieve this goal, we start from a coarse DC estimation (e.g. DensePose) and garment segmentation \cite{Gong2019Graphonomy}, where for each garment we extrapolate the DC of that body part \jimei{a garment may cover multiple body parts. how would you choose?} to fill the garment mask which provides us with an initial DC. We then enforce the geometric consistency between surface normal prediction \cite{Jafarian_2021_CVPR_TikTok} and DC to refine the initial coarse DC by preserving conformality (angle) and isometry (length) with respect to the underlying 3D surface. To ensure that the prediction is temporally coherent we also impose the optical flow consistency between adjacent frames. Figure \ref{fig:teaser} shows the results of our method in swapping textures for a sequence from the TikTok dataset \cite{Jafarian_2021_CVPR_TikTok} and a YouTube video. \tuanfeng{this paragraph can only talk about single image, you may start another paragraph talking about video, also mention that video is trained via one network, and frames are encoded as image feature.}
% from \href{https://youtu.be/3V9vqd1W1gA?t=418}{YouTube}.




\textbf{Third paragraph}\\
Our end-to-end trainable method takes as input a video sequence containing RGB
images of each frame, corresponding garment foreground, the surface normal prediction \cite{Jafarian_2021_CVPR_TikTok}, and initial human DC
coordinates from DensePose \cite{guler2018densepose}, and outputs a high-fidelity  temporally consistent DC coordinate that captures fine wrinkles and the geometry that are faithful to the input image. Our framework "GeoDC" learns the spatial relationship between the surface normal and DC coordinate which guide the network to predict the high-fidelity DC coordinates faithful to the geometry captured in the surface normal. We use a Siamese design of GeoDC to measure the temporal consistency of a pair of consecutive frames %w.r.t optical flow \cite{LucasK81,LucasK85} \jimei{Did you use RAFT? So to cite} from the RGB images.
To that end, our method is self-supervised by
leveraging the geometric correlation between the surface normal and DC coordinates and between frames' temporal consistency. This method does not use any type of ground truth information for the training.
We demonstrate that our method outperforms the state-of-the-art human and dynamic surface DC estimation approaches on both real and rendered images.

\textbf{Forth paragraph}\\
We present five core contributions: (1) a novel formulation that captures the correlation between the surface normal and DC coordinates by maintaining the conformality (angle) and isometry (length), which allows us to
utilize in the wild real videos without any use of ground truth; (2) a design that learns
to predict temporally coherent DC estimation for the frames of a video \tuanfeng{encode the frame by image feature}; (3) incorporating the determinant of jacobian matrix of the predicted DC to prohibit singularity points in the DC coordinate prediction and ensure that the surface normal is pointing
to +\textbf{Z} direction; (4) a novel DC alignment approach in canonical space to evaluate different DC prediction methods; (5) strong qualitative and quantitative prediction on real-world imagery.

\tuanfeng{3) and 4) is weak to me}
\label{sec:intro}

==> cvpr_method_1DExample_Tuanfeng.tex <==
\subsection{\tuanfeng{1D Example: Tuanfeng}}

==> cvpr_method_1DExample_Yasamin.tex <==
\subsection{\yasamin{1D Example: Yasamin}}

To simplify the problem we reduce one dimension and instead of a 3D surface we consider a 1D string on a 2D plane Figure \ref{Fig:straight_line}. The blue line is our unwrapped string. This unwrapped line can represent the U values. Let’s say it starts from 0 and ends to 1. Any point in between has a uniform value based on their location on the line between 0-1.
 

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.475\textwidth]{figures/straight_string.JPG}
  \end{center}
     \vspace{-6mm}
  \caption{The unwrapped straight line can represent a UV coordinate space where the start of the string has a U value of 0 and the end of the string has a value of 1.}
  \label{Fig:straight_line}
  \vspace{-3mm}
\end{figure}

\subsubsection{Experiment1: Straight line along the x axis}

As shown in Figure \ref{Fig:straight_line_exp} let us leave the string straight on the $\textbf{xy}$ plane (geometry graph). Now you can show the u to x graph as well which represents: $\textbf{u} = g(\textbf{x})$ 
As this example the string is straight the graph is a linear graph. Note that in all the figures, the blue line is the actual string on the $\textbf{xy}$ plane (geometric graph). Red arrow again shows the slope of the string on the $\textbf{xy}$ axis. As shown in the (u-x assignment graph), $du = dx$ therefore, $du/dx = 1$.

\begin{figure*}[h]
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/straight_string_experiment.JPG}
  \end{center}
     \vspace{-6mm}
  \caption{The relationship between $\textbf{u}$ and $\textbf{x}$ axis (right diagram) derived from the orientation of the line placement on the $\textbf{xy}$ plane (left diagram). red arrow on the geometry plane represents the slope.}
  \label{Fig:straight_line_exp}
  \vspace{-3mm}
\end{figure*}


\subsubsection{Experiment2: Curved string on the $\textbf{xy}$ plane}

As shown in Figure \ref{Fig:curved_line_exp}, let us leave the string curved on the $\textbf{xy}$ axis (geometry graph). Now you can show the u to x graph as well which represents: $\textbf{u} = g(\textbf{x})$ . As in this example the string is curved the graph is a curved graph with respect to the slopes ($r$) in the geometry graph. For any point on the curved string, there is a slope $r$ that can be represented as angle alpha: 

\begin{align}
r = tan(\alpha) = \frac{sin(\alpha)}{cos(\alpha)}
\end{align}

Then the  $du/dx$ can be computed as follows:

\begin{align}
du = \sqrt{dx^2 + dy^2}
\end{align}

As based on the definition of slope, $dy = r \times dx$, the eq 2 can be rewritten as:

\begin{align}
du = (\sqrt{1 + r^2})~~dx \longrightarrow
\frac{du}{dx} = \sqrt{1 + r^2}
\end{align}

By replacing the eq 1 in eq 3, we can get the relationship between the surface normal (derived from angle $\alpha$) and $\textbf{u}$ coordinate.

\begin{align}
\frac{du}{dx} = \frac{1}{cos~\alpha}
\end{align}

\begin{figure*}[h]
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/curved_string_experiment.JPG}
  \end{center}
     \vspace{-6mm}
  \caption{The relationship between $\textbf{u}$ and $\textbf{x}$ axis (right diagram) derived from the orientation of the line placement on the $\textbf{xy}$ plane (left diagram). Red arrow on the geometry plane represents the slope.}
  \label{Fig:curved_line_exp}
  \vspace{-3mm}
\end{figure*}

==> cvpr_method_1DExample_Yi.tex <==
\subsection{\yi{1D Example: Yi}}

==> cvpr_method_network_temp.tex <==
\subsection{Implementation details}
\label{chapter:framework}

We model $g$ using a 12-layer multi-layer perception, with ReLU \cite{relu} as an activation function after each layer that takes as input a pixel coordinate with positional encoding,  $\gamma(\mathbf{x})$ where $\gamma:\mathds{R}^2\rightarrow\mathds{R}^n$ is Fourier based positional encoding~\cite{tancik2020fourfeat}. We obtain the partial derivative of $g$ by computing the adjacent pixel locations' differences. In the case of processing a video, we use ResNet~\cite{He_2016_CVPR_resnet} to extract per-frame 256 dimensions of image feature $\mathbf{f}_\mathbf{x}$. Our network design is illustrated in Figure \ref{Fig:network} (for image-based UV map prediction) and \ref{Fig:networkvid} (for video-based UV map prediction). To make our prediction scale-invariant, we crop the garments region with $256\times256$ resolution. for the training, we use Adam optimizer \cite{kingma:2015} with batch size 2048 and learning rate $1e−4$. We train our network for 250
epochs, and we find this is usually enough for convergence.
We set  $ \lambda_{\rm prox} = 0.2$, $\lambda_{\rm z} = 0.01 $, and $\lambda_{\rm tmp} = 0.3$
for all the experiments. We test our method with an NVIDIA
V100 GPU and Intel(R) Xeon(R) CPU $E5-2698 v4 @ 2.20GHz$, and implemented our approach
with Pytorch \cite{pytorch}. 

\begin{figure}[t]
\begin{center}
    {\includegraphics[width=0.495\textwidth]{figures/framework2_3.pdf}}\\\vspace{-2mm}
\end{center}
\vspace{-3mm}
   \caption{\textbf{Single image framework.} For each pixel location on a garment $\textbf{p}$, we predict the corresponding location in the Dense Correspondences (DC) canonical space ($\textbf{u}$). By enforcing $\mathcal{L}_{geo}$  we ensure the detailed geometry captured in the surface normal is preserved in the predicted dense correspondence map. To exclude any singularity points happening in the prediction as well as keep the surface normal pointing to +\textbf{Z} direction we also enforce the determinant of the Jacobian matrix to be always negative ( $\mathcal{L}_{jac}$). Finally, we take advantage of the DensePose \cite{guler2018densepose} extrapolation \cite{Telea_inpaint}, to guide our prediction range on the conical space ($\mathcal{L}_{reg}$). }
\label{Fig:network}
\vspace{-5mm}
\end{figure}

\begin{figure*}[h]
\begin{center}
    {\includegraphics[width=1.0\textwidth]{figures/framework6_2.pdf}}\\\vspace{-2mm}
\end{center}
\vspace{-3mm}
   \caption{\textbf{Video framework.} For a pair of frames from a video sequence we ensure the predicted dense correspondences are aligned with the optical flow \cite{LucasK81, LucasK85}. To do so, we pre-compute the correspondences between frame $i$ and $j$ using dense optical flow tracking, which can provide us the warping $W_{i\rightarrow j}$ to warp the prediction of one frame to the other. We then enforce the $\mathcal{L}_{flow}$ to ensure temporal coherency. }
\label{Fig:networkvid}
\vspace{-5mm}
\end{figure*}

% \iffalse
% We design a multilayer perceptron (MLP) \cite{mlp} based network to predict per-pixel dense correspondences of a garment in the input image to the corresponding texture space as shown in Figure \ref{Fig:network}.  Here we discuss the training setup and loss functions both for (1) a single input image and (2) an input video. 

% \noindent\textbf{Single-image training}
% As illustrated in Figure \ref{Fig:network}, for each pixel location $\textbf{p} = (x,y) \in \mathds{R}^2$ in the image space that belongs to the garment of interest, we predict the correspondence $\textbf{u} = (u,v)\in \mathds{R}^2$ in the texture space of the garment. This prediction is parameterized by an MLP $g(\textbf{p}) = \textbf{u}$. We optimize for the parameters of $g$ by minimizing a loss function including the terms $\mathcal{L}_{reg}$, $\mathcal{L}_{geo}$, and $\mathcal{L}_{jac}$ as follows:
% \begin{align}
% \mathcal{L}_{total} = \mathcal{L}_{reg} + \lambda_{geo} \mathcal{L}_{geo} + \lambda_{jac} \mathcal{L}_{jac}, 
% \end{align}

% where $\lambda_{geo}$ and $\lambda_{jac}$ determine how each term is weighted. Based Equation~\ref{eq_res2}, we have a geometry term,
% \begin{align}
% \begin{split}
% \mathcal{L}_{geo}(x,y) =& \|(\frac{\partial u}{\partial x})^2+(\frac{\partial v}{\partial x})^2 - \frac{n_x^2+n_z^2}{n_z^2} \| \\
% +& \|(\frac{\partial u}{\partial y})^2+(\frac{\partial v}{\partial y})^2 - \frac{n_y^2+n_z^2}{n_z^2}\| \\
% +& \|\frac{\partial u}{\partial x}\frac{\partial u}{\partial y}+\frac{\partial v}{\partial x}\frac{\partial v}{\partial y} -\frac{n_xn_y}{n_z^2} \|.
% \end{split}
% \label{eq:jacobian5}
% \end{align}

% In addition on quantitative properties of the partial derivatives, we also notice that $J_g$ should also be positive-definite since the mapping should keep the normal pointing to $+\textbf{Z}$ direction as well as should exclude any singularity points. We use a Jacobian loss to reflect this,
% \begin{equation}
%  \mathcal{L}_{jac}(x,y)
% \begin{cases}
%     -\textbf{det}(J_g(x,y)),& \text{if } \textbf{det}(J_g(x,y)) \leq 0\\
%     0,              & \text{otherwise}
% \end{cases}
% \end{equation}


% Since there can be multiple $(u,v)$ parameterizations (subject to a rotation) that satisfy the constraints of the mapping we are looking for, we regularize our optimization based on some rough initial dense correspondences. Specifically, we use DensePose \cite{guler2018densepose} to obtain an initial per-pixel uv estimates. Since DensePose makes predictions only for the human body, we use a simple extrapolation method~\cite{Telea_inpaint} to extrapolate the predictions to cover the whole garment region resulting in $g'(\textbf{p}) = \textbf{u'}$. 
% %To generate an initial coarse UV for our supervision we first extract the UV from DensePose \cite{guler2018densepose}, and extrapolate \cite{Telea_inpaint} the body part that is most representative of the garment to contain the full garment mask ($g'(\textbf{p}) = \textbf{u'}$ where $\textbf{u'} = (u',v')\in \mathds{R}^2$). For instance, we extrapolate  the DensePose's torso for obtaining a coarse UV of dress and Tshirt instances and DensePose's right upper leg for the skirt. 
% $\mathcal{L}_{reg}$ regularizes our final dense correspondence estimates by staying close to those obtained from DensePose:

% \begin{align}
%     \mathcal{L}_{reg} = \sum_{\textbf{p} \in \mathcal{R}(\textbf{I})}\|g'(\textbf{p})-g(\textbf{p})\|, 
% \end{align}

% \noindent\textbf{Video training} When the input is a video, we extend the MLP based network architecture designed to overfit to a single image to utilize an additional feature vector as shown in Figure \ref{Fig:networkvid}. Specically, we extract features from each RGB frame using the pre-trained ResNet-152 \cite{He_2016_CVPR_resnet} backbone.
% %
% %To achieve a dense correspondence map representative of the local geometry while maintaining the temporal coherency, we train a Siamese structure of our dense correspondence MLP.
% %To guide the network in differentiating between frames of a video, we also extract a feature vector from the RGB image of each frame. 
% This feature vector is concatenated with the pixel locations $\textbf{p}$ and fed to the MLP ($\textit{g}(.)$) to predict the correspondence $\textbf{u}$ in the texture space. When training $\textit{g}(.)$ we introduce an additional flow loss to ensure temporal coherency resulting in the following loss function:
% %The predicted $\textbf{u} = (u,v)\in \mathds{R}^2$ is supervised using $\mathcal{L}_{reg}$, $\mathcal{L}_{geo}$, and $\mathcal{L}_{jac}$ and $\mathcal{L}_{flow}$ as follows: 

% \begin{align}
% \mathcal{L}_{total} = \mathcal{L}_{reg} + \lambda_{geo} \mathcal{L}_{geo} + \lambda_{jac} \mathcal{L}_{jac} + \lambda_{flow} \mathcal{L}_{flow} 
% \end{align}

% To quantify $\mathcal{L}_{flow}$, we first compute the optical flow dense tracking \cite{LucasK81, LucasK85} for the input video and use the flow to warp the predicted dense correspondences from frame $i$ to $j$: $\textbf{u}_{i\rightarrow j}= W_{i\rightarrow j}(\textbf{u}_{i})$. We then define $\mathcal{L}_{flow} $ as:

% \begin{align}
%     \mathcal{L}_{flow} = \sum_{\textbf{p}_{i} \in \mathcal{R}(\textbf{I}_{i})}\|\textbf{u}_{i\rightarrow j}-\textbf{u}_{j}\|, 
% \end{align}

% \fi

% We minimize the following overall loss to learn the UV coordinate from real videos:


% for a single image framework, 



% \noindent\textbf{Architecture} Our MLP has $12$ layers with dimensions of $384,384$ with ReLU \cite{relu} as activation function after each layer. The same architecture is used for image and video input. We refer to the supplementary materials for a detailed network architecture figure.

% We first run human body parsing method~\cite{Gong2019Graphonomy} to extract the mask of the garment of interest. We crop the input image around the mask (for each frame of the video) before starting our approach. To allow our network to learn high-frequency UV coordinates from the 2D image domain, we adopt Random Fourier Feature\cite{tancik2020fourfeat}, $\gamma(x,y): \mathbb{R}^2 \mapsto \mathbb{R}^{?}$, before we input the pixel location into the MLP. 
% The pre-defined proxy map of human $g'$ is extended from DensePose~\cite{guler2018densepose}. Since the map from~\cite{guler2018densepose} is in parts, we adopt the upper-front body (id: $\#$2) for upper body clothes (e.g., shirt, dress); and upper-right leg (id: $\#$9) for lower body clothes (e.g., shorts and trousers). We use ResNet~\cite{he2016deep} to produce an \duygu{fill the dimension} $xx$-dimensional image feature $\mathbf{f}_\mathbf{x}$ for each frame when working with a video input. We crop the garment of interest and resize it to  \duygu{fill the dimension} $x \times x$ when computing the ResNet feature to remove the spatial ambiguity. 
% We obtain optical flow between any two frames from the video via an off-the-shelf approach~\cite{teed2020raft}. 
% \noindent\textbf{Architecture} Our MLP has $x$ layers with dimensions of $a-b-c-d$ with xxx as activation function after each layer. Same architecture are used for image and video input. We refer to the supplementary materials for a detailed network architecture figure.
% \noindent\textbf{Training} We use Adam optimizer~\cite{kingma:2015} with batch size $2048$ and learning rate $10^{-4}$. We train our network for $250$ epochs and we find this is usurall enough for convergence. We set $\lambda_{reg} = 0.2, \lambda_{geo} = 1.0 ,  \lambda_{jac} = 0.01 ,\lambda_{flow} = 0.3$ for all the experiments. We test our method with a NVIDIA V100 GPU and xxx CPU, and implemented our approach with Pytorch~\cite{}. 
%For the dense correspondence network, we train an MLP \cite{mlp} structure and to obtain the dense feature vectors (Figure \ref{Fig:networkvid}), we use the pre-trained ResNet-152 \cite{He_2016_CVPR_resnet} as the feature encoding module.

==> derivate_backup_donotremove.tex <==




Here we are interested in a mapping $\textbf{g}: (x,y) \mapsto (u,v)$ that maps a pixel located at $(x,y)$ in the image to a location $(u,v)$ on the UV space. To study this mapping, we consider its inverse mapping $\textbf{f}: (u,v) \mapsto (x,y)$ that maps a location on the UV space to the image plane (if visible). Since $\textbf{f}$ and $\textbf{g}$ are inverse to each other, according to the \emph{Inverse function theorem}, we have 
\begin{equation}
    J_\textbf{f} \times J_\textbf{g} = \textbf{I},
    \label{eq:jacobian}
\end{equation}
where $J_\ast$ is the Jacobian matrix of a mapping, $\textbf{I}$ is an identity matrix of order 2.

Let us first split $\textbf{f}$ into $\textbf{t}_1: (u,v) \mapsto (\omega_x,\omega_y,\omega_z)$, and $\textbf{t}_2: (\omega_x,\omega_y,\omega_z) \mapsto (x,y)$, where $\textbf{t}_1$ maps a point $\phi = (u,v)$ in UV space to a point $\omega$ over the 3D garment surface and $\textbf{t}_2$ maps $\omega$ to a pixel $\rho = (x,y)$ in the image space.
Let us also assume $\textbf{t}_2$ is an orthogonal camera projection from 3D space to image space, as simple as $\textbf{t}_2(\omega_x,\omega_y,\omega_z) = (\omega_x,\omega_y)$. 

For $J_\textbf{f}$, we have 
\begin{align}
J_\textbf{f} = \begin{bmatrix}
             \frac{\partial x}{\partial u}~~~~\frac{\partial x}{\partial v}\\\\
             \frac{\partial y}{\partial u}~~~~\frac{\partial y}{\partial v}
             \end{bmatrix} = \begin{bmatrix}
             \frac{\partial \omega_x}{\partial u}~~~~\frac{\partial \omega_x}{\partial v}\\\\
             \frac{\partial \omega_y}{\partial u}~~~~\frac{\partial \omega_y}{\partial v}
             \end{bmatrix}.
             \label{eq:jacobian2}
\end{align}
This is because the \emph{chain rule} gives us 
\begin{equation}
    \frac{\partial x}{\partial u} = \frac{\partial x}{\partial \omega_x}\frac{\partial \omega_x}{\partial u} + \frac{\partial x}{\partial \omega_y}\frac{\partial \omega_y}{\partial u} + \frac{\partial x}{\partial \omega_z}\frac{\partial \omega_z}{\partial u}
\end{equation},
and orthogonal camera $\textbf{t}_2$ makes $\frac{\partial x}{\partial \omega_x}=1$ and $\frac{\partial x}{\partial \omega_y}=\frac{\partial x}{\partial \omega_z}=0$, the same for other entries in Equation~\ref{eq:jacobian2}.

To calculate $\frac{\partial \omega_x}{\partial u}$, let us consider a 3D point $\omega \in \mathds{R}^{3} = \textbf{t}_1(\phi)$ on the cloth surface, where $\phi = (u,v)$ on the UV space. We assume the clothes is physically non-stretchable, so the mapping $\textbf{t}_1$ is isometric. This makes
\begin{equation}
    \textbf{u}=\begin{bmatrix}
             \frac{\partial \omega_x}{\partial u}\\\\
             \frac{\partial \omega_y}{\partial u}\\\\
             \frac{\partial \omega_z}{\partial u}
             \end{bmatrix}, \textrm{and} \  \textbf{v}=\begin{bmatrix}
             \frac{\partial \omega_x}{\partial v}\\\\
             \frac{\partial \omega_y}{\partial v}\\\\
             \frac{\partial \omega_z}{\partial v}
             \end{bmatrix}
\end{equation}
forms a tangent plan at point $\omega$ and subject to 
\begin{equation}
    \|\textbf{u}\| = 1,\|\textbf{v}\| = 1, \textbf{u} \perp \textbf{v} \perp \textbf{n},
\end{equation}
where $\textbf{n}$ is the normal direction predicted from the previous step. Without loss of generality, let us assume ${\textbf{u},\textbf{v},\textbf{n}}$ forms a right hand system, i.e., $\textbf{u}\times\textbf{v} = \textbf{n}$. 
Given the fact that $\textbf{n}$ is a unit length vector representing the normal direction, it can be written by its spherical coordinates as
\begin{align}
\textbf{n} = \begin{bmatrix}
             sin\alpha~~sin\beta\\
             cos\alpha\\
             sin\alpha~~cos\beta
             \end{bmatrix}
\end{align},
where $\alpha \in [0,\pi/2]$ and $\beta \in [0,\pi]$ (Figure \ref{Fig:normal_angles}).

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.475\textwidth]{figures/normal_parameterisation.pdf}
  \end{center}
     \vspace{-6mm}
  \caption{The surface normal can be represented by two angles $\alpha$ (the angle between surface normal and y axis) and $\beta$ (the angle between z axis and the projection of surface normal on $\textbf{XZ}$ plane).}
  \label{Fig:normal_angles}
  \vspace{-3mm}
\end{figure}

Mathematically, we can create the following two vector $\mu$ and $\nu$:
\begin{align}
\mu = \begin{bmatrix}
             cos\beta\\
             0\\
             -sin\beta
             \end{bmatrix}
 , 
\nu = \begin{bmatrix}
             -cos\alpha~~sin\beta\\
             sin\alpha\\
             -cos\alpha~~cos\beta
             \end{bmatrix} 
\end{align},
and we have
\begin{equation}
    \|\mu\| = 1,\|\nu\| = 1, \mu \perp \nu \perp \textbf{n} , \mu \times \nu = \textbf{n}.
\end{equation}
Therefore, the 2D plane spanned by ${\textbf{u},\textbf{v}}$ and the 2D plane spanned by ${\mu,\nu}$ should be the same one, which is the tangent plane at point $\omega$. As a result, ${\textbf{u},\textbf{v}}$ is equivalent to ${\mu,\nu}$ subject to a rotation $\theta$ along $\textbf{n}$. So we have
\begin{align}
\begin{split}
\textbf{u} &= \mu cos\theta - \nu sin\theta \\ 
\textbf{v} &= \mu sin\theta + \nu cos\theta.
\end{split}
\end{align}
Therefore
\begin{align}
\begin{split}
\frac{\partial \omega_x}{\partial u}&= cos\theta cos\beta+sin\theta cos\alpha sin\beta\\
\frac{\partial \omega_y}{\partial u}&= -sin\theta sin\alpha \\
\frac{\partial \omega_x}{\partial v}&= sin\theta cos\beta-cos\theta cos\alpha sin\beta\\
\frac{\partial \omega_y}{\partial v}&= cos\theta sin\alpha
\end{split}
\label{eq:jacobian3}
\end{align}


Given Equation~\ref{eq:jacobian} and Equation~\ref{eq:jacobian2}, we have
\begin{align}
    \begin{split}
    \begin{bmatrix}
             \frac{\partial \omega_x}{\partial u}\\\\
             \frac{\partial \omega_y}{\partial u}
    \end{bmatrix} \frac{\partial u}{\partial x} +    \begin{bmatrix}
             \frac{\partial \omega_x}{\partial v}\\\\
             \frac{\partial \omega_y}{\partial v}
    \end{bmatrix} \frac{\partial v}{\partial x} =   \begin{bmatrix}1\\0 \end{bmatrix}
    \\
    \begin{bmatrix}
             \frac{\partial \omega_x}{\partial u}\\\\
             \frac{\partial \omega_y}{\partial u}
    \end{bmatrix} \frac{\partial u}{\partial y} +    \begin{bmatrix}
             \frac{\partial \omega_x}{\partial v}\\\\
             \frac{\partial \omega_y}{\partial v}
    \end{bmatrix} \frac{\partial v}{\partial y} =   \begin{bmatrix}0\\1 \end{bmatrix}   
\end{split}
\label{eq:jacobian4}
\end{align}

Now bringing Equation~\ref{eq:jacobian3} into Equation~\ref{eq:jacobian4}, we solve the linear system as:
\begin{align}
\begin{split}
    \frac{\partial u}{\partial x}&= \frac{ cos\theta}{cos\beta}
    ,\\
    \frac{\partial v}{\partial x}&= \frac{ sin\theta}{cos\beta}
    ,\\
    \frac{\partial u}{\partial y}&= \frac{ cos\theta~~cos\alpha~~sin\beta~~-~~sin\theta~~cos\beta}{sin\alpha~~cos\beta}
    ,\\
    \frac{\partial v}{\partial y}&= \frac{ cos\theta~~cos\beta~~+~~sin\theta~~cos\alpha~~sin\beta}{sin\alpha~~cos\beta}.
    \end{split}
\end{align}
Here $\alpha$ and $\beta$ are from the normal prediction, the only unknown variable is $\theta$. To remove the dependence on $\theta$, we observe,
\begin{align}
\begin{split}
(\frac{\partial u}{\partial x})^2+(\frac{\partial v}{\partial x})^2 ~~= \frac{1}{(cos\beta)^2}
,~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
(\frac{\partial u}{\partial y})^2+(\frac{\partial v}{\partial y})^2 ~~= \frac{(cos\alpha)^2~(sin\beta)^2+ (cos\beta)^2}{(cos\beta)^2~(sin\alpha)^2}
,~~\\
\frac{\partial u}{\partial x}\frac{\partial u}{\partial y}+\frac{\partial v}{\partial x}\frac{\partial v}{\partial y}=\frac{cos\alpha~sin\beta}{sin\alpha~(cos\beta)^2}~~~~~~~~~~~~~~~~~~~~~~~~~~
\end{split}
\label{eq:jacobian5}
\end{align}

Equation~\ref{eq:jacobian5} links the mapping $\textbf{g}: (x,y) \mapsto (u,v)$ with the normal direction for each pixel. It gives us a set of second order derivatives to constrain $\textbf{g}$ with normal information.


==> method_old.tex <==
\section{Method}
\label{sec:method}

\begin{figure*}[th]
\begin{center}

    {\includegraphics[width=1\textwidth]{figures/framework1.pdf}}\\\vspace{-2mm}
\end{center}
\vspace{-3mm}
   \caption{single-view framework.}
\label{Fig:network}
\vspace{-5mm}
\end{figure*}

Consider a mapping $g(\textbf{p}) = \textbf{u}$ that maps a pixel location $\textbf{p} = (p,q) \in \mathds{R}^2$ in the image space that belongs to a garment of the interest to a point $\textbf{u} = (u,v)\in \mathds{R}^2$ in the UV space of the garment as shown in Figure~\ref{Fig:mappings}. The goal of our work is to find such a mapping $g$ that takes into account the local surface geometry denoted by the surface normal predicted at $\mathbf{p}$. We denote the 3D surface normal of $\mathbf{p}$ in the camera space as $\mathbf{N}_\mathbf{p}\in \mathds{S}^2$. % is the 3D surface normal at the 3D point $\mathbf{X} = (x,y,z)\in \mathds{R}^3$ of which projection is $\mathbf{p}$, i.e., $\mathbf{p} = \Pi \mathbf{X}$ where $\Pi$ is the operation of 2D projection. 

Let us define a \textit{conformal} and \textit{isometric} map from the UV texture map to the 3D surface, $f(\mathbf{u}) = \mathbf{X}$. This map is conformal as it preserves angle, and it is isometric as it preserves length. These are the fundamental properties of a texture mapping~\cite{}, stating that the texture is non-stretchable:
\begin{align}
    &{\rm isometric:}~~\left\|f_u\right\| = \left\|f_v\right\| = 1, \nonumber\\ 
    &{\rm conformal:}~~f_u^\mathsf{T} f_v = 0, 
\end{align}
where $f_u$ and $f_v$ are the partial derivatives with respect to $u$ and $v$, respectively. Geometrically, $f_u$ and $f_v$ are the orthogonal tangential vectors on the 3D surface where its cross product forms the surface normal:
\begin{align}
    \widetilde{\mathbf{N}}_{\mathbf{u}} = {f_u} \times {f_v}~~\rightarrow~~ \widetilde{\mathbf{N}}_{\mathbf{p}} = {f_u}(g(\mathbf{p})) \times {f_v}(g(\mathbf{p}))\label{Eq:cross}
\end{align}
where $\widetilde{\mathbf{N}}_{\mathbf{u}}\in \mathds{S}^2$ is the surface normal at $\mathbf{X}$ corresponding to $\mathbf{u}$. $\widetilde{\mathbf{N}}_{\mathbf{p}}$ is the reparametrization of the surface normal with respect to $\mathbf{p}$.

We find the UV mapping $g$ by matching the surface normal $\widetilde{\mathbf{N}}_{\mathbf{p}}$ derived by Equation~(\ref{Eq:cross}) and the surface normal predicted by the image $\mathbf{N}_\mathbf{p}$:
\begin{align}
    \underset{\boldsymbol{\theta}_g,\boldsymbol{\theta}_f}{\operatorname{minimize}} &\sum_{\mathbf{p}} \left\|f_u(g(\mathbf{p}))\times f_v(g(\mathbf{p})) - \mathbf{N}_\mathbf{p}\right\|^2,\nonumber\\
    &{\rm s.t.}~~~\left\|f_u\right\| = \left\|f_v\right\| = 1, f_u^\mathsf{T} f_v = 0, \label{Eq:opt}
\end{align}
where $\boldsymbol{\theta}_g$ and $\boldsymbol{\theta}_f$ are the parameters (neural network weights) of the function $g$ and $f$, respectively.
% Since it is conformal, the surface normal that is the spatial derivative of the surface can be expressed in terms of $(u,v)$:
% \begin{align}
    
% \end{align}

A key challenge of solving Equation~(\ref{Eq:opt}) lies in finding $f$ that requires full 3D reconstruction of the surface. It is an under-constrained system as the depth prediction is often far less unreliable than the surface normal prediction~\cite{yasamin_cvpr}. Instead, we formulate a dual problem that can solve Equation~(\ref{Eq:opt}) effectively without finding $f$, i.e., no 3D reconstruction is needed.

We use two properties. First, we assume orthographic projection, i.e., $(p,q) = (x,y)$. This allows us to express the 3D derivatives using the pixel coordinates:
\begin{align}
    g^{-1}_u = f_u^{1:2}, ~~~g^{-1}_v = f_v^{1:2},
\end{align}
where $f^{1:2}$ is the first two elements ($x,y$) of $f$. $g^{-1}$ is the inverse of $g$ that maps the UV texture map to the pixel coordinate. Second, we derive the derivatives of $g^{-1}$ by using inverse function theorem~\cite{}:
\begin{align}
g^{-1}\circ g(\mathbf{p}) = \mathbf{p} ~~\rightarrow~~\mathbf{J}_{g^{-1}} \mathbf{J}_g = \mathbf{I}_2,
\end{align}
where $\mathbf{J}_g$ is the Jacobian matrix of $g$, and $I_2$ is the $2\times2$ identity matrix. 



---end of HS edit


\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.475\textwidth]{figures/mapping.pdf}
  \end{center}
     \vspace{-6mm}
  \caption{xxx}
  \label{Fig:mappings}
  \vspace{-3mm}
\end{figure}
\subsection{Preliminaries and Assumptions}
Here we are interested in the mapping $g: \textbf{P}(p,q) \mapsto \textbf{U}(u,v)$ that maps a pixel of garment located at $\textbf{P} = (p,q)$ in the image to a location $\textbf{U} = (u,v)$ on the UV space, as shown in Figure~\ref{Fig:mappings}. Given the fact that the image is capturing a garment surface in real world, therefore a 3D garment surface should exist. We denote the mapping from UV space to 3D garment surface as $f: \textbf{U}(u,v) \mapsto \textbf{X}(x,y,z)$, where $\textbf{X}$ is a 3D point on the garment surface. Accordingly, we denote $h: \textbf{X}(x,y,z) \mapsto \textbf{P}(p,q)$, as a camera projection from the 3D space to image plane. Due to the nature that the clothes are made from pieces of non-stretchable garment, we know $f$ is an isometric and conformal mapping. To simplify the problem, we also assume $h$ is an orthogonal camera projection as simple as
\begin{equation}
    h(x,y,z) = (x,y) = (p,q).
    \label{eq:orthogonal}
\end{equation}

%Given a single image of a dressed human $\textbf{I}$, we reconstruct its high fidelity UV, i.e., $\textbf{[u,v]} = g(\mathbf{[x,y]};\mathbf{I})$,
%where $\mathbf{[x,y]} \in \mathds{R}^{2}$ is the $xy$-location in the image, and $\textbf{[u,v]} \in \mathds{R}^{2}$ is the UV at the corresponding location. 

%\input{cvpr_method_1DExample_Yasamin}
% \input{cvpr_method_1DExample_Tuanfeng}
% \input{cvpr_method_1DExample_HyunSoo}
% \input{cvpr_method_1DExample_Duygu}

\subsection{Surface Normal Conditioned UV representation}
\label{sec:NormalvsUV}

Given the normal map predicted from image $I$ through an off-the-shelf normal estimator, e.g., \cite{xx}, for a pixel $\textbf{P}$, we know the normal direction $\textbf{n}_\textbf{P}$ for point $\textbf{X} = f \circ g (\textbf{P})$ on the 3D garment surface. We formulate the mapping $g$ and $f$ as the solution of the following optimization problem:
\begin{align}
\displaystyle \min_{g,f} ~~& \|\frac{\partial}{\partial u} f \circ g (\textbf{P}) \times \frac{\partial}{\partial v} f \circ g (\textbf{P}) -\textbf{n}_\textbf{P}\| \label{eq:optimization_1}\\ 
\textrm{s.t.} ~~& f \textnormal{ is isometric and conformal} \label{eq:optimization_2}\\
& h \circ f \circ g = \textbf{I}_2, \label{eq:optimization_3}
\end{align}
where $\textbf{I}_2$ is an identity mapping of order 2.

Due to Constraint~\ref{eq:optimization_2}, we have 
\begin{align}
    \|\frac{\partial}{\partial u} f \circ g (\textbf{P})\| = 1,  \|\frac{\partial}{\partial v} f \circ g (\textbf{P})\| = 1, \\
    \frac{\partial}{\partial u} f \circ g (\textbf{P}) \cdot \frac{\partial}{\partial v} f \circ g (\textbf{P})= 0. 
\end{align}

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.475\textwidth]{figures/normal_parameterisation.pdf}
  \end{center}
     \vspace{-6mm}
  \caption{The surface normal can be represented by two angles $\alpha$ (the angle between surface normal and y axis) and $\beta$ (the angle between z axis and the projection of surface normal on $\textbf{XZ}$ plane).}
  \label{Fig:normal_angles}
  \vspace{-3mm}
\end{figure}

That means $\frac{\partial}{\partial u} f \circ g (\textbf{P})$ and $\frac{\partial}{\partial v} f \circ g (\textbf{P})$ are perpendicular to each other and forms the tangent plane at $\textbf{X}=f \circ g (\textbf{P})$. Considering $\textbf{n}$ is a unit length vector representing the normal direction, it can be written by its spherical coordinates as
\begin{align}
\textbf{n} = \begin{bmatrix}
             sin\alpha~~sin\beta\\
             cos\alpha\\
             sin\alpha~~cos\beta
             \end{bmatrix}
\end{align},
where $\alpha \in [0,\pi/2]$ and $\beta \in [0,\pi]$ (Figure \ref{Fig:normal_angles}). The tangent plane can also be spanned by the two vectors following the latitude direction ($\mu$) and the longitude direction ($\nu$), i.e.,
\begin{align}
\mu = \begin{bmatrix}
             cos\beta\\
             0\\
             -sin\beta
             \end{bmatrix}
 , 
\nu = \begin{bmatrix}
             -cos\alpha~~sin\beta\\
             sin\alpha\\
             -cos\alpha~~cos\beta
             \end{bmatrix} .
\end{align}
Since the tangent plane is unique, frame $[\frac{\partial}{\partial u} f \circ g (\textbf{P}),\frac{\partial}{\partial v} f \circ g (\textbf{P})]$ and $[\nu,\mu]$ is equivalent subject to a rotation $\theta$ along $\textbf{n}$, as shown in Figure~\ref{Fig:normal_angles}. Therefore we can rewrite our optimization into an unconditional form,
\begin{align}
\displaystyle \min_{g,f} ~~& \| [\frac{\partial}{\partial u} f \circ g (\textbf{P}) ~~ \frac{\partial}{\partial v} f \circ g (\textbf{P})]^T-\textbf{Rot}(\theta)[\nu ~~ \mu]^T\|. \label{eq:opt_un}
\end{align}

We further reshape it to 
\begin{align}
\begin{split}
%\displaystyle \min_{g,f} ~~& \| \begin{bmatrix} \frac{\partial p}{\partial u}\\\\ \frac{\partial q}{\partial u}\\\\ \frac{\partial z}{\partial u} \end{bmatrix} - (\mu cos\theta - \nu sin\theta) \| \\ + &\| \begin{bmatrix} \frac{\partial p}{\partial v}\\\\ \frac{\partial q}{\partial v}\\\\ \frac{\partial z}{\partial v} \end{bmatrix} - (\mu sin\theta + \nu cos\theta) \|
\displaystyle \min_{g,f} ~~& \| [ \frac{\partial p}{\partial u} ~~ \frac{\partial q}{\partial u} ~~ \frac{\partial z}{\partial u}]^T - (\mu cos\theta - \nu sin\theta) \| \\ + &\| [ \frac{\partial p}{\partial v} ~~ \frac{\partial q}{\partial v} ~~ \frac{\partial z}{\partial v}]^T - (\mu sin\theta + \nu cos\theta) \|
\end{split}
\end{align}

Combining with Equation~\ref{eq:orthogonal}, we know $f \circ g(p,q) =(p,q,z)$. Let us drop the $z$-channel and have $f_* = f_{[1:2]}$, which takes only the first two dimensions from $f$. As a result, $f_*$ and $g$ are inverse to each other. Therefore, the above optimization can be rewritten as,
\begin{align}
\begin{split}
\displaystyle \min_{g,f_*} ~~& \| \frac{\partial p}{\partial u} - (cos\theta cos\beta+sin\theta cos\alpha sin\beta)\| \\
+&\| \frac{\partial q}{\partial u} - (-sin\theta sin\alpha)\| \\
+&\| \frac{\partial p}{\partial v} - (sin\theta cos\beta-cos\theta cos\alpha sin\beta)\| \\
+&\| \frac{\partial q}{\partial v} - (cos\theta sin\alpha)\| \\
\end{split}
\end{align}

Since $g$ and $f_*$ are inverse to each other, according to the \emph{Inverse function theorem}, we have 
\begin{equation}
    J_{f_*} \times J_{g} = \textbf{I}_2,
    \label{eq:jacobian}
\end{equation}
where $J_\ast$ is the Jacobian matrix of a mapping, $\textbf{I}_2$ is an identity matrix of order 2. This converts the Jacobian of $f_*$, $\frac{\partial p,q}{\partial u,v}$, into the Jacobian of $g$, $\frac{\partial u,v}{\partial p,q}$. So we have our optmization directly on $g$ as follow,
\begin{align}
\begin{split}
\displaystyle \min_{g} ~~& \| \frac{\partial u}{\partial p} - \frac{ cos\theta}{cos\beta}\| \\
+&\| \frac{\partial v}{\partial p} - \frac{ sin\theta}{cos\beta}\| \\
+&\| \frac{\partial u}{\partial q} - \frac{ cos\theta~~cos\alpha~~sin\beta~~-~~sin\theta~~cos\beta}{sin\alpha~~cos\beta}\| \\
+&\| \frac{\partial v}{\partial q} - \frac{ cos\theta~~cos\beta~~+~~sin\theta~~cos\alpha~~sin\beta}{sin\alpha~~cos\beta}\|. \\
\end{split}
\end{align}

Note that $\alpha$ and $\beta$ are from the normal direction which are known, the only unknown variable is $\theta$. To remove the dependence on $\theta$, we perform elimination by calculating the products of the derivatives. This further convert our optimization into 
\begin{align}
\begin{split}
\displaystyle \min_{g} ~~& \|(\frac{\partial u}{\partial p})^2+(\frac{\partial v}{\partial p})^2 - \frac{1}{(cos\beta)^2} \| \\
+& \|(\frac{\partial u}{\partial q})^2+(\frac{\partial v}{\partial q})^2 - \frac{(cos\alpha)^2~(sin\beta)^2+ (cos\beta)^2}{(cos\beta)^2~(sin\alpha)^2}\| \\
+& \|\frac{\partial u}{\partial p}\frac{\partial u}{\partial q}+\frac{\partial v}{\partial p}\frac{\partial v}{\partial q} -\frac{cos\alpha~sin\beta}{sin\alpha~(cos\beta)^2} \|.
\end{split}
\label{eq:jacobian5}
\end{align}

Equation~\ref{eq:jacobian5} links the mapping $g: (p,q) \mapsto (u,v)$ with the normal direction for each pixel. It gives us a set of products of the derivatives to constrain $g$ with normal information.




% \subsection{Implementation}

% \tuanfeng{not ready yet}
% \tuanfeng{to discuss: regularization loss, network, etc.}
% \tuanfeng{no need to mention PD map? this is just a visualization}

% and as follows we can generate a PDmap (Partial Derivative map) from both UV and surface normal. the consistency between these two maps supervises our UV refinement using surface normal. Each of the following equations represent each of the 3 channels in these PDmaps where the left side of the equations are the PDmaps derived from UV and the right side of the equations represent the PDmaps derived from surface normal:

% The equation above can be rewritten in the form of $\textbf{PD}_{uv}$ and  $\textbf{PD}_{n}$ as follows:

% \begin{align}
% \textbf{PD}_{uv}([\textbf{x,y}])~=~\begin{bmatrix}
%              (\frac{\partial \mathbf{u}}{\partial x})^2+(\frac{\partial \mathbf{v}}{\partial x})^2
%              \\\\
%              (\frac{\partial \mathbf{u}}{\partial y})^2+(\frac{\partial \mathbf{v}}{\partial y})^2
%              \\\\
%              \frac{\partial \mathbf{u}}{\partial x}\frac{\partial \mathbf{u}}{\partial y}+\frac{\partial \mathbf{v}}{\partial x}\frac{\partial \mathbf{v}}{\partial y}
%              \end{bmatrix}
%  \\
% \textbf{PD}_{n}([\textbf{x,y}])~=~\begin{bmatrix}
%              \frac{1}{(cos\beta)^2}
%              \\\\
%              \frac{(cos\alpha)^2~(sin\beta)^2+ (cos\beta)^2}{(cos\beta)^2~(sin\alpha)^2}
%              \\\\
%              \frac{cos\alpha~sin\beta}{sin\alpha~(cos\beta)^2}
%              \end{bmatrix}
% \end{align}

% Finally the geometric loss is computed as follows:

% \begin{align}
%     \mathcal{L}_{geo} = \sum_{\mathbf{I}_i\in \mathcal{D}_s}\sum_{\mathbf{[x,y]} \in \mathcal{R}(\mathbf{I}_i)}\|\lambda \textbf{PD}_{uv}([\textbf{x,y}])-\textbf{PD}_{n}([\textbf{x,y}])\|^2
% \end{align}

% Where where $\mathcal{D}_s$ is the real data dataset, and $\lambda$ is a scaling factor to take care of the rotation ambiguity cause by $\theta$. In practice $\lambda$ is pre-computed on the ground-truth template and is used as an approximated scaling factor for all the real data images.

% \subsection{Temporal Consistency}

\input{cvpr_method_network.tex}
